Optimized Markov Chain Monte Carlo for Signal Detection in MIMO Systems: an Analysis of Stationary Distribution and Mixing Time

In this paper we introduce an optimized Markov Chain Monte Carlo (MCMC) technique for solving the integer least-squares (ILS) problems, which include Maximum Likelihood (ML) detection in Multiple-Input Multiple-Output (MIMO) systems. Two factors contribute to the speed of finding the optimal solution by the MCMC detector: the probability of the optimal solution in the stationary distribution, and the mixing time of the MCMC detector. Firstly, we compute the optimal value of the "temperature" parameter, in the sense that the temperature has the desirable property that once the Markov chain has mixed to its stationary distribution, there is polynomially small probability ($1/\mbox{poly}(N)$, instead of exponentially small) of encountering the optimal solution. This temperature is shown to be at most $O(\sqrt{SNR}/\ln(N))$, where $SNR$ is the signal-to-noise ratio, and $N$ is the problem dimension. Secondly, we study the mixing time of the underlying Markov chain of the proposed MCMC detector. We find that, the mixing time of MCMC is closely related to whether there is a local minimum in the lattice structures of ILS problems. For some lattices without local minima, the mixing time of the Markov chain is independent of $SNR$, and grows polynomially in the problem dimension; for lattices with local minima, the mixing time grows unboundedly as $SNR$ grows, when the temperature is set, as in conventional wisdom, to be the standard deviation of noises. Our results suggest that, to ensure fast mixing for a fixed dimension $N$, the temperature for MCMC should instead be set as $\Omega(\sqrt{SNR})$ in general. Simulation results show that the optimized MCMC detector efficiently achieves approximately ML detection in MIMO systems having a huge number of transmit and receive dimensions.

==> Conclusion/Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}
In this paper we have introduced a new approach to solving the integer least-squares problem using the Markov Chain Monte Carlo method called MCMC sampling. The proposed MCMC method will, unlike simulated annealing techniques, have a fixed temperature parameter in all the iterations, with the property that after the Markov chain has mixed, the probability of encountering the optimal solution is only polynomial small (i.e. not exponentially small). To the authors knowledge, this is a novel way of looking at the minimization problem, and the optimal value of temperature parameter for this approach has been calculated. From the analysis of the MCMC method and the simulation results we can see there is a trade-off between faster mixing time of the Markov chain versus the speed of finding the optimal solution in the steady-state distribution. We also analyzed the mixing time of the underlying Markov chains. It is also interesting to extend this work to MIMO system with channel codes in future works.
%
%In this paper, we study the mixing time of Markov Chain Monte Carlo (MCMC) for the integer least-square optimization problem. It is found that the mixing time of MCMC for the integer least-square problem depends on the structure of the underlying lattice. More specifically, the mixing time of MCMC is found to be closely related to whether there is a local minimum in the lattice structure of the integer least-square problem. For some lattices, the mixing time of the Markov chain is independent of the signal-to-noise ratio; while for some lattices, the mixing time is correlated with the signal-to-noise ratio. We also derive the probability that there exist local minima in an integer least-square problem, which can be as high as $\frac{1}{3}-\frac{1}{\sqrt{5}}+\frac{2\arctan(\sqrt{\frac{5}{3}})}{\sqrt{5}\pi}$. Both theoretical and empirical results suggest that to ensure fast mixing for the MCMC for the integer least-square problem, the temperature for MCMC should often grow as the signal-noise-ratio increases. 

==> Finding_optimal_alpha/Backup_mean_steady_state.tex <==
\section{Mean of $\pi_{-\oneb}$}
In the following section we compute the expected value of the steady-state probabilities of the states. More specifically we are examining the probability of state $\sb = -\oneb$, denoted $\pi_{-\oneb}$ (recall that we assumed that $-\oneb$ is transmitted symbol vector). This calculation has a lot in common with the one given in Section \ref{sec:P_error}. Note that
%\begin{eqnarray}
%\begin{subequations}
\begin{align*}
\pi_{-\oneb} & = \frac{e^{-\frac{1}{2\alpha^2}\left\|\yb+\sqrt{\frac{\SNR}{N}}\Hb \oneb\right\|^2}}
{\sum_s e^{-\frac{1}{2\alpha^2}\left\|\yb+\sqrt{\frac{\SNR}{N}}\Hb \sb\right\|^2}} \\
& = \frac{e^{-\frac{1}{2\alpha^2}\left\|\upsib\right\|^2}}
{\sum_\sb e^{-\frac{1}{2\alpha^2}\left\|\upsib+\sqrt{\frac{\SNR}{N}}\Hb(\sb-\oneb)\right\|^2}} \\
& = \frac{e^{-\frac{1}{2\alpha^2}\left\|\upsib\right\|^2}}
{\sum_{\delta} e^{-\frac{1}{2\alpha^2}\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb \delb\right\|^2}} \\
& = \frac{1} {\sum_{\delb} e^{-\frac{1}{2\alpha^2}\left(
\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2-\|\upsib\|^2\right)}} \ ,
\end{align*}
%\end{subequations}
%\end{eqnarray}
where $\delb$ is a vector of zeros and ones.

Now, by Jensen
\begin{subequations}
\begin{align}
\Ec \left\{ \pi_{-\oneb} \right\} & \geq \frac{1}{\Ec \left\{ \frac{1}{\Ec \left\{ \pi_{-\oneb}\right\} }\right\} } \\
 & =  
\frac{1}{\Ec \left\{ \sum_{\delta} e^{-\frac{1}{2\alpha^2}\left(
\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb \delb\right\|^2-\left\|\upsib\right\|^2\right)} \right\}} \\
& = \frac{1}
{\sum_{\delta} \Ec \left\{ e^{-\frac{1}{2\alpha^2}\left(
\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb \delb\right\|^2-\left\|\upsib\right\|^2\right) }\right\} } \\
& = \frac{1}{1+\sum_{\delb \neq 0}
\left(\frac{1}{1+4\frac{\SNR\left\|\delb\right\|^2}{N}
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})}\right)^{N/2}} \label{Eq:Jensen_part4} \\
& = \frac{1}{1+\sum_{i=1}^N\left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+4\frac{\SNR i}{N}
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})}\right)^{N/2}} \ .
\end{align}
\end{subequations}
In \eqref{Eq:Jensen_part4} have used Lemma \ref{lem:g-i}. While it is possible to focus on the linear and sublinear terms in the
above summation separately, to give conditions for $\Ec \left\{ \pi_{-\oneb} \right\}$ to have
the form of $1/\mbox{poly}(N)$, we will be interested in the exact
exponent of the poly and so we need a more accurate estimate. To do
this we shall use saddle point integration. To this end, note that
\begin{align*}
\left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+4\frac{\SNR i}{N} \frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})}\right)^{N/2} \\ 
= e^{N H(\frac{i}{N})-\frac{N}{2}\ln\left(1+4\frac{\SNR i}{N} \frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})\right)} \ ,
\end{align*}
again $H(\cdot)$ represents the entropy in ``nats''. And so the summation can be
approximated as a Stieltjes integral:
\begin{subequations}
\begin{align}
& \sum_{i=1}^N\left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+4\frac{\SNR i}{N}
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})}\right)^{N/2} \\
& = N\sum_{i=1}^Ne^{N H(\frac{i}{N})-\frac{N}{2}\ln\left(1+4\frac{\SNR i}{N}
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})\right)}\frac{1}{N} \\
& = N\int_0^1e^{N H(x)-\frac{N}{2}\ln\left(1+4\SNR
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})x\right)}dx \\
& = N\int_0^1e^{N H(x)-\frac{N}{2}\ln\left(1+\beta x\right)}dx \ ,
\end{align}
\end{subequations}
where we have defined $\beta \triangleq 4\SNR
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})$. 

For large $N$, this is a saddle point integral and can be approximated
by the formula
\be
\int_0^1e^{N f(x)}dx \approx \sqrt{\frac{2\pi}{N|f''(x_0)|}}e^{N f(x_0)} \ , 
\label{Eq:saddlepoint}
\ee
where $x_0$, is the saddle point of $f(\cdot)$, i.e.,$f'(x_0) = 0.$
In our case,
\[ f(x) = -x\ln x-(1-x)\ln(1-x)-\frac{1}{2}\ln(1+\beta x) \ , \]
and so
\[ f'(x) = \ln\frac{1-x}{x}-\frac{1}{2}\frac{\beta}{1+\beta x} \ . \]
In general, it is not possible to solve for $f'(x_0) = 0$ in closed
form. However, in our case, if we assume that $\beta = 4\SNR
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})\gg 1$ (as will be the case
since the SNR grows at least logarithmically),
then it is not too hard to verify that the saddle point is given by
\be
x_0 = e^{-\frac{\beta}{2}} \ .
\ee
And hence
\begin{equation*}
\begin{split}
f(x_0) & = -e^{-\frac{\beta}{2}}\ln e^{-\frac{\beta}{2}} -(1-e^{-\frac{\beta}{2}})\ln(1-e^{-\frac{\beta}{2}}) \\
& \quad - \frac{1}{2}\ln(1+\beta e^{-\frac{\beta}{2}}) \\
& \approx
\frac{\beta}{2}e^{-\frac{\beta}{2}}+e^{-\frac{\beta}{2}}-\frac{1}{2} \beta e^{-\frac{\beta}{2}} \\
& = e^{-\frac{\beta}{2}} \ ,
\end{split}
\end{equation*}
and further plugging $x_0$ into 
%\[ f''(x) = -\frac{1}{x}-\frac{1-x}+\frac{1}{2}\frac{\beta^2}{(1+\beta
%  x)^2}, \]
\[ f''(x) = -\frac{1}{x} -\frac{1}{1-x}-\frac{1}{2}\frac{\beta^2}{(1+\beta x)^2} \ , \]
yields
\be
f''(x_0) \approx -e^{\frac{\beta}{2}}-1+\frac{1}{2}\beta^2 \approx
-e^{\frac{\beta}{2}} \ . 
\ee
Replacing these into the saddle point expression in \eqref{Eq:saddlepoint} show that
\be
\sum_{i=1}^N \left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+4\frac{\SNR i}{N}
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})}\right)^{N/2} \approx 
\sqrt{2\pi/N} \exp{\left(N e^{-\frac{\beta}{2}}-\frac{\beta}{4}\right)} \ . 
\ee

We want $\Ec \left\{ \pi_{-\oneb} \right\}$ to behave as $\frac{1}{N^\zeta}$ and so this means
that we want the above expression to behave as $N^{\zeta}$. Let us
take
\[ e^{Ne^{-\frac{\beta}{2}}} = N^{\zeta} \ . \]
Solving for $\beta$ yields
\be 
\beta = 2\ln N -\ln\ln N -\ln\zeta .
\ee
Incidentally, this choice of $\beta$ yields
\be
e^{-\frac{\beta}{4}} \approx \frac{1}{\sqrt{N}}.
\ee
Finally, this choice of $\beta$ means that we have
\[ 4\SNR \frac{1}{\alpha^2}(1-\frac{1}{\alpha^2}) = 
2\ln N -\ln\ln N -\ln\zeta \ , \]
and so we have the following result

\begin{lemma}[Mean of $\pi_{-\oneb}$] If $\alpha$ is chosen such that 
\be
\frac{\alpha^2}{1-\frac{1}{\alpha^2}} = \frac{4\SNR}
{2\ln N -\ln\ln N -\ln\zeta} \ ,
\ee
then
\be
\Ec \left\{\pi_{-\oneb} \right\} \geq N^{-\zeta} \ .
\ee
\end{lemma}

==> Package_setup.tex <==
\usepackage{amssymb,amsmath,amsthm}
\usepackage{mathrsfs} %For the \mathscr font style

%For the \mathpzc font style
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{2 <-> pzcmi8t}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> [1.5] pzcmi8t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\usepackage{MnSymbol}
%\usepackage[T!]{fontenc}
%\usepackage[latin1]{inputenc}

%\usepackage[bottom]{footmisc}
\usepackage[latin1]{inputenc}
\usepackage[english]{babel}
\usepackage[]{subfig}

%\usepackage[numbered,framed]{mcode}
\usepackage[]{color}

%\usepackage{epsfig,graphics}
\usepackage{epic,eepic,epsfig,graphics}
%\usepackage[dvips]{graphicx}

\usepackage{cite}
% fix citations to be IEEE style
\def\citepunct{], [}
\def\citedash{]--[}
%\def\citedash{-}

\usepackage{color}						%M added
\definecolor{red}{rgb}{1,0,0}	%M added
%Command: \textbf{\textcolor{red}{RED TEXT}}

%\usepackage{epsfig,psfrag,pst-all,verbatim}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}


%------Alex's Macros---------------------
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\stexp}{\mbox{$\mathsf{E}$}}    % Statistical Expectation operator
\newcommand{\poly}{\text{Poly}}
\newcommand{\LL}{\mathcal{L}}
\def\qed{\quad \vrule height6.5pt width6pt depth0pt} %Nifty end proof sign
%------Babak's Macros---------------------
\newcommand{\ovr}{\overline}
\newcommand{\no}{\noindent}
\def\ker{{\rm ker}\,}
\def\dim{{\rm dim}\,}
\newcommand{\st}{\stackrel{J}{\approx}}
\newcommand{\stt}{\stackrel{I}{\approx}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beqr}{\begin{eqnarray}}
\newcommand{\eeqr}{\end{eqnarray}}
\newcommand{\beqrx}{\begin{eqnarray*}}
\newcommand{\eeqrx}{\end{eqnarray*}}
\newcommand{\ba}{\left[ \begin{array}}
\newcommand{\ea}{\\ \end{array} \right]}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\lb}{\label}
\newcommand{\rf}{\ref}
\newcommand{\ov}{\bar}
\newcommand{\td}{(t-1)}
\newcommand{\xx}{t-1}
\newcommand{\tl}{\tilde}
\newcommand{\qd}{\hfill{\qed}}
\def\qed{{\ \vrule width 2.5mm height 2.5mm \smallskip}}
%------...end there--------------------------

\def\xb{{\bf x}}
\def\sb{{\bf s}}
\def\yb{{\bf y}}
\def\zb{{\bf z}}
\def\bb{{\bf b}}
\def\vb{{\bf v}}
\def\db{{\bf d}}
\def\hb{{\bf h}}
\def\upsib{\boldsymbol{\upsilon}}
\def\delb{\boldsymbol{\delta}}

\def\Hb{{\bf H}}
\def\Ib{{\bf I}}
\def\Ab{{\bf A}}
\def\Bb{{\bf B}}

\def\Rbb{\mathbb{R}}
\def\Nc{\mathcal{N}}
\def\bigO{\mathcal{O}}
\def\Ec{\mathcal{E}}
\def\Sc{\mathcal{S}}
\def\Hc{\mathcal{H}}

\def\hs{\mathpzc{h}}
\def\Ss{\mathpzc{S}}
\def\As{\mathpzc{A}}

\def\vec{\text{vec}}
\def\SNR{\mbox{SNR}}

\def\oneb{\text{\boldmath $1$}}
\def\zerob{\text{\boldmath $0$}}
\def\squeeze{\itemsep=0pt\parskip=0pt} 
